On the Convergence to a Global Solution of Shuffling-Type Gradient Algorithms

Stochastic gradient descent (SGD) algorithm is the method of choice in many machine learning tasks thanks to its scalability and efficiency in dealing with large-scale problems. In this paper, we focus on the shuffling version of SGD which matches the mainstream practical heuristics. We show the convergence to a global solution of shuffling SGD for a class of non-convex functions under over-parameterized settings. Our analysis employs more relaxed non-convex assumptions than previous literature. Nevertheless, we maintain the desired computational complexity as shuffling SGD has achieved in the general convex setting.

==> import.tex <==
% \usepackage[subpreambles=true]{standalone}

% For commenting
% \usepackage{changes}


% Recommended, but optional, packages for figures and better typesetting:
% \usepackage{microtype}
\usepackage{graphicx}
%\usepackage{subfigure}
\usepackage{booktabs} % for professional tables
% \usepackage{amsmath}
% \usepackage{amsfonts} 


\usepackage[flushleft]{threeparttable}


\usepackage{epsf}
\usepackage{fancyhdr}
\usepackage{graphics}
\usepackage{graphicx}
\usepackage{psfrag}
\usepackage{microtype}
%\usepackage{subfigure}
%\usepackage{mathtools, algorithmic}

%\usepackage[linesnumbered,ruled]{algorithm2e}% http://ctan.org/pkg/algorithm2e
%\DontPrintSemicolon
\usepackage{color}
% \usepackage{amssymb,amsmath,amsthm}


% \usepackage{amsthm}
\usepackage{amsfonts}
\usepackage{amsmath}
\usepackage{amssymb,bbm}

\usepackage{algorithm}
\usepackage{algorithmic}



\usepackage{caption,subcaption}
\captionsetup{font=footnotesize}
\usepackage{sidecap}
\sidecaptionvpos{figure}{c}

% hyperref makes hyperlinks in the resulting PDF.
% If your build breaks (sometimes temporarily if a hyperlink spans a page)
% please comment out the following usepackage line and replace
% \usepackage{icml2018} with \usepackage[nohyperref]{icml2018} above.
\usepackage{url}
\usepackage{hyperref}

% Attempt to make hyperref and algorithmic work together better:
% \newcommand{\theHalgorithm}{\arabic{algorithm}}

\newcommand{\strongconvex}{\mu}
\newcommand{\smooth}{L_1}
\newcommand{\smoothprior}{L_2}
\newcommand{\subgaussian}{\sigma}
\newcommand{\barFn}{\bar{F}_n}
\newcommand{\KL}{\mathbf{KL}}
\newcommand{\OT}{\mathbf{OT}}
\newcommand{\UOT}{\mathbf{UOT}}
\newcommand{\diag}{\textnormal{diag}}
%
% \newtheorem{assumption}{Assumption}
% \newtheorem{remark}{Remark}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\setlength{\textwidth}{\paperwidth}
%\addtolength{\textwidth}{-6cm}
%\setlength{\textheight}{\paperheight}
%\addtolength{\textheight}{-4cm}
%\addtolength{\textheight}{-1.1\headheight}
%\addtolength{\textheight}{-\headsep}
%\addtolength{\textheight}{-\footskip}
%\setlength{\oddsidemargin}{0.5cm}
%\setlength{\evensidemargin}{0.5cm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\long\def\comment#1{}
\comment{
% text margin
\setlength{\topmargin}{0 in}
\setlength{\textwidth}{5.5 in}
\setlength{\textheight}{8 in}
\setlength{\oddsidemargin}{0.5 in}
}

% \newtheorem{observation}{Observation}
% \newtheorem{lemma}{Lemma}
% \newtheorem{theorem}{Theorem}
% \newtheorem{proposition}{Proposition}
% \newtheorem{definition}{Definition}
% \newtheorem{corollary}{Corollary}%opening


% \theoremstyle{plain}
% \newtheorem{theorem}{Theorem}[section]
% \newtheorem{proposition}[theorem]{Proposition}
% \newtheorem{lemma}[theorem]{Lemma}
% \newtheorem{corollary}[theorem]{Corollary}
% \theoremstyle{definition}
% \newtheorem{definition}[theorem]{Definition}
% \newtheorem{assumption}[theorem]{Assumption}
% % \theoremstyle{remark}
% \newtheorem{remark}[theorem]{Remark}


% \newtheorem{conjecture}{Conjecture}%opening


%\newtheorem{assumption}{Assumption}
%\newtheorem{conjecture}{Conjecture}
\newenvironment{assumptionprime}[1]
  {\renewcommand{\theassumption}{\ref{#1}$'$}%
   \addtocounter{assumption}{-1}%
   \begin{assumption}}
  {\end{assumption}}
\newcommand{\cheeger}{\mathfrak{h}}

\def\argmin{\textnormal{arg} \min}
\def\st{\textnormal{s.t.}}
\def\sgn{\texttt{sign}}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}

\def\TM{\texttt{T}}
\def\OT{\textnormal{OT}}
\def\TW{\textnormal{TW}}
\def\TSW{\textnormal{TSW}}
\newcommand{\Br}{\mathbb{R}}
\newcommand{\one}{\textbf{1}}
\newcommand{\zero}{\textbf{0}}

\def\GW{{\mathcal{GW}}}

\def\GTW{{\mathcal{GW}_{T}}}
\def\TGW{{\mathcal{GW}_{T}}}

\def\FGTW{{\mathcal{GW}_{T_f}}}
\def\FTGW{{\mathcal{GW}_{T_f}}}
\def\SFGTW{{\mathcal{GW}_{T_f}^2}}
\def\SFTGW{{\mathcal{GW}_{T_f}^2}}
\def\RFGTW{{\widehat{\mathcal{GW}}_{T_f}}}
\def\RFTGW{{\widehat{\mathcal{GW}}_{T_f}}}
\def\SRFGTW{{\widehat{\mathcal{GW}}_{T_f}^2}}
\def\SRFTGW{{\widehat{\mathcal{GW}}_{T_f}^2}}

\def\DGTW{{\mathcal{GW}_{T_d}}}
\def\DTGW{{\mathcal{GW}_{T_d}}}
\def\SDGTW{{\mathcal{GW}_{T_d}^2}}
\def\SDTGW{{\mathcal{GW}_{T_d}^2}}
\def\RDGTW{{\widehat{\mathcal{GW}}_{T_d}}}
\def\RDTGW{{\widehat{\mathcal{GW}}_{T_d}}}
\def\SRDGTW{{\widehat{\mathcal{GW}}_{T_d}^2}}
\def\SRDTGW{{\widehat{\mathcal{GW}}_{T_d}^2}}

\def\FlowTreeGW{\textsf{Flow-TreeGW}}
\def\DepthTreeGW{\textsf{Depth-TreeGW}}
\def\EntropicGW{\textsf{EntropicGW}}
\def\VarEntropicGW{\textsf{Var-EntropicGW}}
\def\SlicedGW{\textsf{SlicedGW}}


\def\RR{\mathbb{R}}
\def\DD{\mathbb{D}}
\def\NN{\mathbb{N}}
\def\PP{\mathbb{P}}
\def\MM{\mathbb{M}}
\def\SS{\mathbb{S}}
\def\EE{\mathbb{E}}
\def\FF{\mathbb{F}}
\def\TT{\mathbb{T}}
\def\XX{\mathbb{X}}
\def\QQ{\mathbb{Q}}
\def\FF{\mathbb{F}}

\def\Ff{\mathcal{F}}
\def\Hh{\mathcal{H}}
\def\Gg{\mathcal{G}}
\def\Ee{\mathcal{E}}
\def\Pp{\mathcal{P}}
\def\Ss{\mathcal{S}}
\def\Ww{\mathcal{W}}
\def\Ff{\mathcal{F}}
\def\Rr{\mathcal{R}}
\def\Nn{\mathcal{N}}
\def\Xx{\mathcal{X}}
\def\Tt{\mathcal{T}}
\def\Mm{\mathcal{M}}
\def\Qq{\mathcal{Q}}
\def\Uu{\mathcal{U}}
\def\Yy{\mathcal{Y}}

\def\aA{\mathbf{a}}
\def\bB{\mathbf{b}}
\def\xX{\mathbf{x}}
\def\yY{\mathbf{y}}
\def\uU{\mathbf{u}}
\def\vV{\mathbf{v}}
\def\pP{\mathbf{p}}
\def\tT{\mathbf{t}}
\def\gG{\mathbf{g}}
\def\pP{\mathbf{p}}
\def\qQ{\mathbf{q}}
\def\lmb{\mathbf{\lambda}}



\def\wW{\mathbf{w}}
\def\rR{\mathbf{r}}
\def\sS{\mathbf{s}}

\graphicspath{{./image/}}

\newcommand{\argmax}{\mathop{\arg \max}}
\newcommand{\br}{\mathbb{R}}
\newcommand{\bs}{\mathbb{S}}
\newcommand{\bn}{\mathbb{N}}
\newcommand{\ba}{\begin{array}}
\newcommand{\ea}{\end{array}}
\newcommand{\ACal}{\mathcal{A}}
\newcommand{\BCal}{\mathcal{B}}
\newcommand{\ZCal}{\mathcal{Z}}
\newcommand{\FCal}{\mathcal{F}}
\newcommand{\RCal}{\mathcal{R}}
\newcommand{\XCal}{\mathcal{X}}
\newcommand{\bp}{\mathbb{P}}
\newcommand{\bq}{\mathbb{Q}}
\newcommand{\NCal}{\mathcal{N}}
\newcommand{\indc}{\mathbb{I}}
\newcommand{\UCal}{\mathcal{U}}
\newcommand{\red}{\color{red}}
\newcommand{\Rspace}{\mathbb{R}}
\newcommand{\bigO}{\mathcal{O}}
\newcommand{\bigOtil}{\widetilde{\mathcal{O}}}
\newcommand{\mydefn}{:=}
\newcommand{\widgraph}[2]{\includegraphics[keepaspectratio,width=#1]{#2}}

\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\genecomment}[1]{{\bf{{\blue{{TEAM --- #1}}}}}}

% infinity/sup/max norm
\newcommand{\mnorm}[1]{\|{#1}\|_{\scriptscriptstyle \infty}}




\newcommand{\lstar}{\ind_\star}
\newcommand{\scalartwo}{b}
\newcommand{\remainder}{\varepsilon}
\newcommand{\myfrac}[2]{\ensuremath{\frac{#1}{#2}}}
\newcommand{\Mtil}{\widetilde{M}}
\newcommand{\PseudoND}{\Mtil_{n,d}}
\newcommand{\vMF}{\emph{vMF}}
\newcommand{\scale}{\ensuremath{\kappa}}
\newcommand{\location}{\ensuremath{\eta}}
\newcommand{\ones}{\mathbf{1}}
%\newcommand{\diag}{\textbf{diag}}

\newcommand{\argminE}{\mathop{\mathrm{argmin}}}   

\newcommand{\at}[2][]{#1|_{#2}}



\newcommand{\alglinelabel}{%
  \addtocounter{ALC@line}{-1}% Reduce line counter by 1
  \refstepcounter{ALC@line}% Increment line counter with reference capability
  \label% Regular \label
}

==> sections/redundant.tex <==
\begin{thm}
Assumptions~\ref{ass_lowerbound_fi}, \ref{ass_Lsmooth_fi}, \ref{ass_PL_fi}, \ref{ass_general_bounded_variance}. Choose $\eta_t \leq \frac{1}{2L \sqrt{3 \Theta + 2}}$. 
\end{thm}

Analysis. For $i \in [n]$, we have
\allowdisplaybreaks
\begin{align*}
    f( w_0^{(t+1)} ; i )  & \overset{\eqref{eq:Lsmooth}}{\leq}   f( w_0^{(t)} ; i ) + \nabla f( w_0^{(t)} ; i )^{\top}(w_0^{(t+1)} - w_0^{(t)}) + \frac{L}{2}\norms{w_0^{(t+1)} - w_0^{(t)}}^2 \\
    %
    &\overset{\tiny\eqref{eq:fact2}}{=} f( w_0^{(t)} ; i ) - \eta_t \nabla f( w_0^{(t)} ; i )^\top \left( \frac{1}{n} \sum_{i=0}^{n-1} \nabla f (w_j^{(t)} ; \pi^{(t)} (j + 1) ) \right) \\ 
    & \qquad  + {~} \frac{L \eta_t^{2}}{2} \left \|  \frac{1}{n}\sum_{j=0}^{n-1} \nabla f (w_j^{(t)} ; \pi^{(t)} (j + 1) ) \right\|^2 \\
    %
    & \overset{\tiny(a)}{=}   f( w_0^{(t)} ; i ) - \frac{\eta_t}{2} \norms{ \nabla f( w_0^{(t)} ; i ) }^2 + \frac{\eta_t}{2} \left \| \nabla f( w_0^{(t)} ; i )  - \frac{1}{n}\sum_{j=0}^{n-1} \nabla f (w_j^{(t)} ; \pi^{(t)} (j + 1) ) \right\|^2 \\
    & \qquad  - {~} \frac{\eta_t}{2} \left( 1 - L\eta_t  \right) \left\| \frac{1}{n}\sum_{j=0}^{n-1} \nabla f (w_j^{(t)} ; \pi^{(t)} (j + 1) ) \right\|^2 \\
    %
    & \overset{\tiny(b)}{\leq}   f( w_0^{(t)} ; i ) - \frac{\eta_t}{2} \norms{ \nabla f( w_0^{(t)} ; i ) }^2 + \frac{\eta_t}{2} \left \| \nabla f( w_0^{(t)} ; i )  - \frac{1}{n}\sum_{j=0}^{n-1} \nabla f (w_j^{(t)} ; \pi^{(t)} (j + 1) ) \right\|^2 \\
    % 
    &= f( w_0^{(t)} ; i ) - \frac{\eta_t}{2} \norms{ \nabla f( w_0^{(t)} ; i ) }^2 \\
    & \qquad + \frac{\eta_t}{2} \left \| \left( \nabla f( w_0^{(t)} ; i ) - \nabla F( w_0^{(t)} ) \right) + \left( \nabla F( w_0^{(t)} ) - \frac{1}{n}\sum_{j=0}^{n-1} \nabla f (w_j^{(t)} ; \pi^{(t)} (j + 1) ) \right) \right\|^2 \\
    % 
    & \overset{\tiny(c)}{\leq} f( w_0^{(t)} ; i ) - \frac{\eta_t}{2} \norms{ \nabla f( w_0^{(t)} ; i ) }^2 + \eta_t \left \| \nabla f( w_0^{(t)} ; i ) - \nabla F( w_0^{(t)} ) \right\|^2  \\
    & \qquad + \eta_t \left \| \frac{1}{n}\sum_{j=0}^{n-1} \nabla f (w_0^{(t)} ; \pi^{(t)} (j + 1) ) - \frac{1}{n}\sum_{j=0}^{n-1} \nabla f (w_j^{(t)} ; \pi^{(t)} (j + 1) )  \right\|^2 \\
    % 
    & \leq f( w_0^{(t)} ; i ) - \frac{\eta_t}{2} \norms{ \nabla f( w_0^{(t)} ; i ) }^2 + \eta_t \left \| \nabla f( w_0^{(t)} ; i ) - \nabla F( w_0^{(t)} ) \right\|^2  \\
    & \qquad + \eta_t \frac{1}{n}\sum_{j=0}^{n-1} \left \|  \nabla f (w_0^{(t)} ; \pi^{(t)} (j + 1) ) - \nabla f (w_j^{(t)} ; \pi^{(t)} (j + 1) )  \right\|^2 \\
    % 
    & \overset{\tiny\eqref{eq:Lsmooth_basic}}{\leq} f( w_0^{(t)} ; i ) - \frac{\eta_t}{2} \norms{ \nabla f( w_0^{(t)} ; i ) }^2 + \eta_t \left \| \nabla f( w_0^{(t)} ; i ) - \nabla F( w_0^{(t)} ) \right\|^2  \\
    & \qquad + \eta_t L^2 \frac{1}{n}\sum_{j=0}^{n-1} \left \|  w_0^{(t)} - w_j^{(t)}  \right\|^2, \tagthis \label{eq_main_001}
\end{align*}
where (\textit{a}) follows from $u^{\top}v = \frac{1}{2}(\norms{u}^2 + \norms{v}^2 - \norms{u - v}^2)$; (\textit{b}) follows from the fact that $\eta_t \leq \frac{1}{2L \sqrt{3 \Theta + 2}} \leq \frac{1}{L}$; and (\textit{c}) follows from $\|u + v \|^2 \leq 2 \| u \|^2 + 2 \| v \|^2$. 

\lam{Not sure if term $- \frac{\eta_t}{4} \left\| \frac{1}{n}\sum_{j=0}^{n-1} \nabla f (w_j^{(t)} ; \pi^{(t)} (j + 1) ) \right\|^2$ could be useful since we also have $\eta_t \leq \frac{1}{2L \sqrt{3 \Theta + 2}} \leq \frac{1}{2L}$.}

Taking the average from $i = 1,\dots, n$ and adding $-F_*$ to both sides of \eqref{eq_main_001}, we have
\begin{align*}
    [ F(w_0^{(t+1)}) - F_* ] & \leq [ F ( w_0^{(t)} ) - F_* ] - \frac{\eta_t}{2} \frac{1}{n} \sum_{i=1}^{n} \norms{ \nabla f( w_0^{(t)} ; i ) }^2 \\
    & \qquad + \eta_t \frac{1}{n} \sum_{i=1}^{n} \left \| \nabla f( w_0^{(t)} ; i ) - \nabla F( w_0^{(t)} ) \right\|^2 + \eta_t L^2 \frac{1}{n}\sum_{j=0}^{n-1} \left \|  w_0^{(t)} - w_j^{(t)}  \right\|^2 \\
    % 
    & \overset{\tiny\eqref{eq:ncvx_keybound1}}{\leq} [ F ( w_0^{(t)} ) - F_* ] - \frac{\eta_t}{2} \frac{1}{n} \sum_{i=1}^{n} \norms{ \nabla f( w_0^{(t)} ; i ) }^2 \\
    & \qquad + \eta_t \frac{1}{n} \sum_{i=1}^{n} \left \| \nabla f( w_0^{(t)} ; i ) - \nabla F( w_0^{(t)} ) \right\|^2 + \eta_t^3 L^2 \left[ \left( 3 \Theta + 2 \right) \|   \nabla F ( w_0^{(t)}) \|^2 + 3 \sigma^2 \right] \\
    %
    & \overset{\tiny(d)}{\leq} [ F ( w_0^{(t)} ) - F_* ] - \frac{\eta_t}{4} \frac{1}{n} \sum_{i=1}^{n} \norms{ \nabla f( w_0^{(t)} ; i ) }^2 \\
    & \qquad + \eta_t \frac{1}{n} \sum_{i=1}^{n} \left \| \nabla f( w_0^{(t)} ; i ) - \nabla F( w_0^{(t)} ) \right\|^2 + 3 \eta_t^3 L^2 \sigma^2 \\
    % 
    & \overset{\tiny\eqref{eq:PL_fi}}{\leq} [ F ( w_0^{(t)} ) - F_* ] - \frac{\eta_t \mu}{2} \frac{1}{n} \sum_{i=1}^{n} [ f( w_0^{(t)} ; i ) - f_i^{*} ] \\
    & \qquad + \eta_t \frac{1}{n} \sum_{i=1}^{n} \left \| \nabla f( w_0^{(t)} ; i ) - \nabla F( w_0^{(t)} ) \right\|^2 + 3 \eta_t^3 L^2 \sigma^2 \\
    % 
    & \overset{\tiny\eqref{eq_loss_great_01}}{\leq} [ F ( w_0^{(t)} ) - F_* ] - \frac{\eta_t \mu}{2} [ F ( w_0^{(t)} ) - F_* ] \\
    & \qquad + \eta_t \frac{1}{n} \sum_{i=1}^{n} \left \| \nabla f( w_0^{(t)} ; i ) - \nabla F( w_0^{(t)} ) \right\|^2 + 3 \eta_t^3 L^2 \sigma^2, 
\end{align*}
where (\textit{d}) follows since $\| \nabla F ( w_0^{(t)}) \|^2 \leq \frac{1}{n} \sum_{i=1}^{n} \norms{ \nabla f( w_0^{(t)} ; i ) }^2$ and $\eta_t \leq \frac{1}{2L \sqrt{3 \Theta + 2}}$. 



\subsection{Convex}

\begin{ass}\label{ass_convex}
Suppose that $f(\cdot; i)$ is convex for all $i \in [n]$, i.e.,
\begin{equation}\label{eq:convex}
f(w ; i)  - f(w' ; i) \geq \langle \nabla f(w' ; i),w - w' \rangle, \quad \forall w, \hat{w} \in \R^d.
\end{equation}
\end{ass}

Assumptions~\ref{ass_Lsmooth_fi} and \ref{ass_convex} imply 
\begin{align*}
    \| \nabla f ( w; i ) \|^2 \leq 2L [f(w;i) - f_i^{*}], \quad \forall w \in \R^d, \tagthis \label{eq_smooth_convex}
\end{align*}
where $f_i^* = \min_{w \in \mathbb{R}^d} f ( w ; i )$, $i \in [n]$. 

\begin{ass}\label{ass_Lipschitz_fi}
Suppose that $f(\cdot; i)$ is $M$-Lipschitz continuous for all $i \in [n]$, i.e. there exists a constant $M \in (0, +\infty)$ such that:
\begin{equation}\label{eq:Lipschitz}
| f(w;i) - \nabla f(\hat{w} ;i) | \leq M \norms{ w - \hat{w}}, \quad \forall w, \hat{w} \in \R^d. 
\end{equation}
\end{ass}

\begin{thm}\label{thm_convex_01}
Let $\{w^{(t)}_i\}$ be the sequence generated by Algorithm~\ref{sgd_replacement} with $\eta_i^{(t)} = \frac{\eta_t}{n}  = \frac{\eta}{n}$, with $0 < \eta \leq \frac{n}{2L}$.
Then, under Assumptions~\ref{ass_lowerbound_fi}, \ref{ass_Lsmooth_fi}, \ref{ass_opt_set}, and \ref{ass_convex}, we have ...
\end{thm}

\begin{proof}
From the update $w_{i+1}^{(t)} := w_{i}^{(t)} - \eta_i^{(t)} \nabla f ( w_i^{(t)} ; \pi^{(t)} ( i + 1 ) )$ in Algorithm~\ref{sgd_replacement} with $\eta_i^{(t)} := \frac{\eta_t}{n}$,  for $i \in [n]$, we have
\begin{align*}
    w_{i}^{(t)} = w_{i-1}^{(t)} - \frac{\eta_t}{n} \nabla f ( w_{i-1}^{(t)} ; \pi^{(t)} (i)) = w_{0}^{(t)} - \frac{\eta_t}{n} \sum_{j=0}^{i-1} \nabla f ( w_{j}^{(t)} ; \pi^{(t)} (j + 1)). \tagthis \label{update_shuffling_01}
\end{align*}
Hence, 
\begin{align*}
    w_{0}^{(t+1)} = w_{n}^{(t)} = w_{0}^{(t)} - \frac{\eta_t}{n} \sum_{j=0}^{n-1} \nabla f ( w_{j}^{(t)} ; \pi^{(t)} (j + 1)). \tagthis \label{update_shuffling_02}
\end{align*}

Let $w^* \in W^*$. We have, 
\begin{align*}
    \| w_{i}^{(t)} - w^* \|^2 & \overset{\eqref{update_shuffling_01}}{=} \| w_{i-1}^{(t)} - w^* \|^2 - \frac{2 \eta_t}{n}\langle \nabla f ( w_{i-1}^{(t)} ; \pi^{(t)} (i)) , w_{i-1}^{(t)} - w^*  \rangle + \frac{\eta_t^2}{n^2} \| \nabla f ( w_{i-1}^{(t)} ; \pi^{(t)} (i))  \|^2 \\
    &\overset{\eqref{eq:convex}\eqref{eq_smooth_convex}}{\leq} \| w_{i-1}^{(t)} - w^* \|^2 - \frac{2 \eta_t}{n} \left[ f ( w_{i-1}^{(t)} ; \pi^{(t)} (i)) - f_{\pi^{(t)} (i)}^* \right] \\ & \qquad + \frac{2L\eta_t^2}{n^2} \left[ f ( w_{i-1}^{(t)} ; \pi^{(t)} (i)) - f_{\pi^{(t)} (i)}^* \right] \\
    & \leq \| w_{i-1}^{(t)} - w^* \|^2 - \frac{\eta_t}{n} \left[ f ( w_{i-1}^{(t)} ; \pi^{(t)} (i)) - f_{\pi^{(t)} (i)}^* \right], 
\end{align*}
where the last inequality follows since $\eta_t \leq \frac{n}{2L}$. Summing $i = 1,\dots,n$, we have
\begin{align*}
    \| w_{n}^{(t)} - w^* \|^2 & \leq \| w_{0}^{(t)} - w^* \|^2 - \eta_t  \frac{1}{n} \sum_{i=1}^{n} \left[ f ( w_{i-1}^{(t)} ; \pi^{(t)} (i)) - f_{\pi^{(t)} (i)}^* \right] \\
    %
    & \leq \| w_{0}^{(t)} - w^* \|^2 - \eta_t  \frac{1}{n} \sum_{i=1}^{n} \left[ f ( w_{i-1}^{(t)} ; \pi^{(t)} (i)) - f ( w_{0}^{(t)} ; \pi^{(t)} (i)) \right] \\
    & \qquad - \eta_t  \frac{1}{n} \sum_{i=1}^{n} \left[  f ( w_{0}^{(t)} ; \pi^{(t)} (i)) - f_{\pi^{(t)} (i)}^*  \right] \\
    %
    & \overset{\tiny\eqref{eq_loss_great_01}}{\leq} \| w_{0}^{(t)} - w^* \|^2 - \eta_t  \frac{1}{n} \sum_{i=1}^{n} \left[ f ( w_{i-1}^{(t)} ; \pi^{(t)} (i)) - f ( w_{0}^{(t)} ; \pi^{(t)} (i)) \right] \\
    & \qquad - \eta_t  \left[  F ( w_{0}^{(t)} ) - F_*  \right] 
\end{align*}

Note that $w_{n}^{(t)} = w_{0}^{(t+1)} = \tilde{w}_{t}$.

\end{proof}

\section{New Redundant 02}

% \begin{ass}\label{ass_basic}
% Assume that problem \eqref{ERM_problem_01} satisfies the following conditions:
% \begin{enumerate}[$($i$)$] 
% \item $F_{*} := \inf_{w\in\R^d}F(w) > -\infty$.
% \item $f(\cdot; i)$ is $L$-smooth for all $i \in [n]$, i.e. there exists a constant $L \in (0, +\infty)$ such that:
% \begin{equation}\label{eq:Lsmooth_basic}
% \norms{ \nabla f(w;i) - \nabla f(\hat{w} ;i)} \leq L \norms{ w - \hat{w}}, \quad \forall w, \hat{w} \in \R^d. 
% \end{equation}
% \end{enumerate}
% \end{ass}

\begin{ass}\label{ass_lowerbound_fi}
Suppose that $f_i^{*} := \inf_{w\in\R^d}f(w;i) > -\infty$, $i \in [n]$. 
\end{ass}

\begin{ass}\label{ass_Lsmooth_fi}
Suppose that $f(\cdot; i)$ is $L$-smooth for all $i \in [n]$, i.e. there exists a constant $L \in (0, +\infty)$ such that:
\begin{equation}\label{eq:Lsmooth_basic}
\norms{ \nabla f(w;i) - \nabla f(\hat{w} ;i)} \leq L \norms{ w - \hat{w}}, \quad \forall w, \hat{w} \in \R^d. 
\end{equation}
\end{ass}


Note that Assumption~\ref{ass_lowerbound_fi} is required in any algorithm to guarantee the well-definedness of \eqref{ERM_problem_01}.
Assumption~\ref{ass_Lsmooth_fi} is standard in gradient-type methods.
Hence, we refer to Assumptions~\ref{ass_lowerbound_fi} and \ref{ass_Lsmooth_fi} as the standard assumptions required throughout the paper.
Assumption \ref{ass_Lsmooth_fi} implies that the objective function $F$ is also $L$-smooth. 
Moreover, as proven in \citep{nesterov2004}, we have for $i \in [n]$, 
\begin{equation}\label{eq:Lsmooth}
f(w; i) \leq f(\hat{w}; i) + \iprods{\nabla f(\hat{w}; i), w - \hat{w}} + \frac{L}{2}\norms{w - \hat{w}}^2, \quad \forall w, \hat{w} \in \R^d.
\end{equation}

\begin{ass}\label{ass_PL_fi}
Suppose that $f(\cdot; i)$ satisfies PL inequality for some constant $\mu \in (0,+\infty)$ such that
\begin{equation}\label{eq:PL_fi}
\norms{ \nabla f(w;i) }^2 \geq 2 \mu [f(w;i) - f_i^{*}], \quad \forall w \in \R^d, 
\end{equation}
where $f_i^{*} := \min_{w\in\R^d}f(w;i)$. 
\end{ass}

\begin{ass}\label{ass_general_bounded_variance}
There exists two constants $\Theta \in [0, +\infty)$ and $\sigma \in (0, +\infty)$ such that
\begin{equation}\label{eq:general_bounded_variance}
    \frac{1}{n} \sum_{i=1}^n \norms{\nabla f(w; i) - \nabla F(w)}^2 \leq \Theta \| \nabla F(w) \|^2 \ + \ \sigma^2, \quad \forall w \in \R^d. 
\end{equation}
\end{ass}

Note that 
\begin{align*}
    F_* &= \min_{w \in \mathbb{R}^d} F ( w )  = \min_{w \in \mathbb{R}^d} \left(\frac{1}{n}\sum_{i=1}^n f_i (w) \right)= \frac{1}{n} \min_{w \in \mathbb{R}^d} \left(\sum_{i=1}^n f_i (w) \right) \\
    &\geq \frac{1}{n} \sum_{i=1}^n \min_{w \in \mathbb{R}^d} \left( f_i (w) \right) = \frac{1}{n} \sum_{i=1}^n f_i^*. \tagthis \label{eq_loss_great_01}
\end{align*}


\begin{ass}\label{ass_general_bounded_gradient}
There exists two constants $M \in (0, +\infty)$ and $N \in (0, +\infty)$ \lam{$N \in (2\mu, +\infty)$ using Assumption~\ref{ass_PL_fi}} such that
\begin{equation}\label{eq:general_bounded_gradient}
    \frac{1}{n} \sum_{i=1}^n \norms{\nabla f(w; i) }^2 \leq M \| \nabla F(w) \|^2 + N [ F(w) - F_*], \quad \forall w \in \R^d, 
\end{equation}
where $F_{*} := \min_{w\in\R^d} F(w)$.
\end{ass}


\lam{We need $N > 2 \mu$ if we also assume PL for each $f(w;i)$.}

Note that for any global solution $w_*$ of $F$ and if $F$ is $L$-smooth, then $\forall w \in \R^d$, 
\begin{align*}
    \frac{1}{n} \sum_{i=1}^n \norms{\nabla f(w; i) }^2 & \leq M \| \nabla F(w) \|^2 + N [ F(w) - F_*] \\
    & \leq ML^2 \| w - w_* \|^2 + \frac{NL}{2} \| w - w_* \|^2 \\
    & \leq L \left( LM + \frac{N}{2} \right) \| w - w_* \|^2,  \tagthis \label{eq:general_bounded_gradient_02}
\end{align*}
which is average $L \left( M + \frac{N}{2} \right)$-smooth of $F$ at $w_*$ if $\nabla f(w_*;i) = 0$, $i \in [n]$. 

If if $\nabla f(w_*;i) \neq 0$, $i \in [n]$, we have for $\alpha > 0$,
\begin{align*}
    \frac{1}{n} \sum_{i=1}^n \norms{\nabla f(w; i) }^2 & = \frac{1}{n} \sum_{i=1}^n \norms{(\nabla f(w_*; i) - \nabla f(w; i) ) - \nabla f(w_*; i) }^2 \\
    & \geq \frac{1}{1 + \alpha} \frac{1}{n} \sum_{i=1}^n \| \nabla f(w_*; i) - \nabla f(w; i) \|^2 - \frac{1}{\alpha} \frac{1}{n} \sum_{i=1}^n \| \nabla f(w_*; i) \|^2. 
\end{align*}

Hence, 
\begin{align*}
    \frac{1}{n} \sum_{i=1}^n \| \nabla f(w; i) - \nabla f(w_*; i) \|^2 & \leq (1 + \alpha) \frac{1}{n} \sum_{i=1}^n \norms{\nabla f(w; i) }^2 + \frac{1 + \alpha}{\alpha} \frac{1}{n} \sum_{i=1}^n \| \nabla f(w_*; i) \|^2 \\
    & \overset{\tiny\eqref{eq:general_bounded_gradient_02}}{\leq} L (1 + \alpha) \left( LM + \frac{N}{2} \right) \| w - w_* \|^2 + \frac{1 + \alpha}{\alpha} \frac{1}{n} \sum_{i=1}^n \| \nabla f(w_*; i) \|^2. 
\end{align*}

We also have for $\alpha > 0$,
\begin{align*}
    \frac{1}{n} \sum_{i=1}^n \norms{\nabla f(w; i) }^2 & = \frac{1}{n} \sum_{i=1}^n \norms{(\nabla f(w_*; i) - \nabla f(w; i) ) - \nabla f(w_*; i) }^2 \\
    & \leq \left( 1 + \frac{1}{\alpha} \right) \frac{1}{n} \sum_{i=1}^n \| \nabla f(w; i) - \nabla f(w_*; i) \|^2 + (1 + \alpha) \frac{1}{n} \sum_{i=1}^n \| \nabla f(w_*; i) \|^2. 
\end{align*}

\begin{ass}\label{ass_general_bounded_weight_00}
There exists three constants $\gamma \in (0, +\infty)$, $\beta \in (0, +\infty)$, $P \in (0, +\infty)$, and $Q \in (0, +\infty)$ such that
\begin{equation}\label{eq:general_bounded_weight_00}
    \gamma \left( \inf_{\hat{w} \in \mathcal{W}_*} \| w - \hat{w} \|^2 \right) + \beta \left( \frac{1}{n} \sum_{i=1}^n \norms{\nabla f(w; i) }^2 \right) \leq P \| \nabla F(w) \|^2 + Q [ F(w) - F_*], \quad \forall w \in \R^d, 
\end{equation}
where $F_{*} := \min_{w\in\R^d} F(w)$, and $\hat{w}$ is in the optimal solution set $\mathcal{W}_*$. 
\end{ass}

From this assumption, we have
\begin{align*}
    - \| \nabla F(w) \|^2 \leq - \frac{\gamma}{P} \left( \inf_{\hat{w} \in \mathcal{W}_*} \| w - \hat{w} \|^2 \right) - \frac{\beta}{P} \left( \frac{1}{n} \sum_{i=1}^n \norms{\nabla f(w; i) }^2 \right) +  \frac{Q}{P} [ F(w) - F_*], \quad \forall w \in \R^d, 
\end{align*}

\begin{ass}\label{ass_general_bounded_weight}
There exists three constants $\gamma \in (0, +\infty)$, $P \in (0, +\infty)$, and $Q \in (0, +\infty)$ such that
\begin{equation}\label{eq:general_bounded_weight}
    \gamma \left( \inf_{\hat{w} \in \mathcal{W}_*} \| w - \hat{w} \|^2 \right) \leq  \frac{1}{n} \sum_{i=1}^n \norms{\nabla f(w; i) }^2 + P \| \nabla F(w) \|^2 + Q [ F(w) - F_*], \quad \forall w \in \R^d, 
\end{equation}
where $F_{*} := \min_{w\in\R^d} F(w)$, and $\hat{w}$ is in the optimal solution set $\mathcal{W}_*$. 
\end{ass}

Using Assumption~\ref{ass_general_bounded_weight} with Assumption~\ref{ass_general_bounded_gradient}, for any global solution $w_*$ of $F$ and if $F$ is $L$-smooth, then from \eqref{eq:general_bounded_gradient_02} we have $\forall w \in \R^d$, 
\begin{align*}
    \gamma \left( \inf_{\hat{w} \in \mathcal{W}_*} \| w - \hat{w} \|^2 \right) &\leq L \left( LM + \frac{N}{2} \right) \| w - w_* \|^2 + L \left( L P + \frac{Q}{2} \right) \| w - w_* \|^2 \\
    & = L \left( L(M + P) + \frac{N+Q}{2} \right) \| w - w_* \|^2.
\end{align*}

From \eqref{eq:general_bounded_weight}, we have $\forall w \in \R^d$,
\begin{align*}
    - \| \nabla F(w) \|^2 \leq - \frac{\gamma}{P} \left( \inf_{\hat{w} \in \mathcal{W}_*} \| w - \hat{w} \|^2 \right) + \frac{1}{P} \frac{1}{n} \sum_{i=1}^n \norms{\nabla f(w; i) }^2 + \frac{Q}{P} [ F(w) - F_*]. \tagthis \label{ass_general_bounded_weight_02}
\end{align*}

\begin{ass}\label{ass_general_bounded_gradient_02}
There exists two constants $P \in (0, +\infty)$ and $Q \in (0, +\infty)$ such that $\forall w, w' \in \R^d$, 
\begin{equation}\label{eq:general_bounded_gradient}
    \frac{1}{n} \sum_{i=1}^n \norms{\nabla f(w; i) - \nabla f(w'; i) }^2 \leq P \| \nabla F(w) - \nabla F(w') \|^2 + Q [ F(w) - F(w')]. 
\end{equation}
\end{ass}

Assumption~\ref{ass_general_bounded_gradient_02} implies Assumption~\ref{ass_general_bounded_gradient} when $w' = w_*$. 

Assumption~\ref{ass_general_bounded_gradient} is motivated from \cite{Bottou2018}. If $F$ satisfies PL condition, that is, $\| \nabla F( w ) \|^2 \geq 2 \tau [F(w) - F_*]$, for some $\tau > 0$, then Assumption~\ref{ass_general_bounded_gradient} implies
\begin{align*}
    \frac{1}{n} \sum_{i=1}^n \norms{\nabla f(w; i) }^2 \leq M \| \nabla F(w) \|^2 + N [ F(w) - F_*] \leq \left( M + \frac{N}{2 \tau} \right) \| \nabla F(w) \|^2,  
\end{align*}
which is Strong Growth Condition. Note that the assumption on PL for each individual $f(w;i)$ cannot imply Strong Growth Condition since PL for each individual $f(w;i)$ cannot imply the PL of $F$. PL condition for $F$ is very strong since it implies that every stationary point of $F$ is also a global optimal solution. 

If $F$ satisfies PL condition with some parameter $\tau > 0$, then we have
\begin{align*}
      2 \tau [F(w) - F_*] \leq \| \nabla F( w ) \|^2 \leq \frac{1}{n} \sum_{i=1}^{n} \| \nabla f ( w ; i ) \|^2,
\end{align*}
but note that
\begin{align*}
    [F(w) - F_*] \overset{\tiny\eqref{eq_loss_great_01}}{\leq} \frac{1}{n} \sum_{i=1}^{n} [f(w;i) - f_i^{*}].
\end{align*}

Hence, we cannot conclude anything. 

If $w_*$ is a global optimal solution of $F$, then with overparameterized setting, we assume that $\sigma_*^2 = \frac{1}{n} \sum_{i=1}^n \norms{\nabla f(w_*; i) }^2 \leq \mathcal{O}(\varepsilon)$ for some small $\varepsilon > 0$ ($\sigma_*$ is the lowest value among $w_* \in \mathcal{W}_*$). Therefore, Assumption \ref{ass_general_bounded_gradient} is reasonable since $\| \nabla F(w_*) \|^2 \leq \mathcal{O}(\varepsilon)$ and $[ F(w_*) - F_*] \leq \mathcal{O}(\varepsilon)$. If $\hat{w}$ is not a global solution of $F$ but a stationary point of $F$, then $\| \nabla F(\hat{w}) \|^2 \leq \mathcal{O}(\varepsilon)$ but $[ F(\hat{w}) - F_*]$ is away from $\mathcal{O}(\varepsilon)$, so $\frac{1}{n} \sum_{i=1}^n \norms{\nabla f(\hat{w}; i) }^2$ is also away from $\mathcal{O}(\varepsilon)$ since
\begin{align*}
    2\mu [ F(w) - F_*] & \leq 2\mu \frac{1}{n} \sum_{i=1}^n [ f(w;i) - f_i^{*} ] \\ & \leq \frac{1}{n} \sum_{i=1}^n \norms{\nabla f(w; i) }^2 \leq M \| \nabla F(w) \|^2 + N [ F(w) - F_*]. \tagthis \label{eq:general_bounded_gradient_PL}
\end{align*}
Hence, $\hat{w}$ is not a stationary point of each individual function $f(w;i)$, $i \in [n]$. 


From \eqref{eq:general_bounded_gradient}, we have
\begin{align*}
    - \| \nabla F(w) \|^2 \leq - \frac{1}{M} \frac{1}{n} \sum_{i=1}^n \norms{\nabla f(w; i) }^2 + \frac{N}{M} [ F(w) - F_*]. \tagthis \label{eq:general_bounded_gradient_02}
\end{align*}

Hence, using Assumption~\ref{ass_PL_fi}, we have
\begin{align*}
    - \| \nabla F(w) \|^2 & \leq - \frac{2 \mu}{M} \frac{1}{n} \sum_{i=1}^n [f(w;i) - f_i^{*}] + \frac{N}{M} [ F(w) - F_*] \\
    & \overset{\tiny\eqref{eq_loss_great_01}}{\leq} - \frac{2\mu}{M} [F(w) - F_*] + \frac{N}{M} [ F(w) - F_*] = - \frac{1}{M} (2 \mu - N) [F(w) - F_*]. 
\end{align*}

Hence, if $2 \mu > N$, then it could imply PL for $F$. 

\begin{defn}\label{defn_opt_comp_set}
We define
\begin{align*}
    W_i^* = \{ w \in \mathbb{R}^d : f ( w ; i ) = f_i^* = \min_{w \in \mathbb{R}^d} f ( w ; i ) \} \ , \ i = 1,\dots,n. 
\end{align*}
and the optimal set
\begin{align*}
    W^* = \bigcap_{i=1}^n W_i^*. 
\end{align*}
\end{defn}

\begin{ass}\label{ass_opt_set}
The optimal set $W^*$ is nonempty, that is, there exists $w^*$ such that $w^* \in W^* \neq \varnothing$. 
\end{ass}

\begin{algorithm}[hpt!]
   \caption{(Generic Shuffling-Type Gradient Algorithm for Solving \eqref{ERM_problem_01})}\label{sgd_replacement}
\begin{algorithmic}[1]
   \STATE {\bfseries Initialization:} Choose an initial point $\tilde{w}_0\in\dom{F}$.
   \FOR{$t=1,2,\cdots,T $}
   \STATE Set $w_0^{(t)} := \tilde{w}_{t-1}$;
   \STATE Generate any permutation  $\pi^{(t)}$ of $[n]$ (either deterministic or random);
   \FOR{$i = 1,\cdots, n$}
    \STATE Update $w_{i}^{(t)} := w_{i-1}^{(t)} - \eta_i^{(t)} \nabla f ( w_{i-1}^{(t)} ; \pi^{(t)} ( i ) )$; 
   \ENDFOR
   \STATE Set $\tilde{w}_t := w_{n}^{(t)}$;
   \ENDFOR
\end{algorithmic}
\end{algorithm} 

\subsection{Non-Convex}

Let us first state the following facts.
\begin{itemize}
\item Let $w_{*}$ be a stationary point of $F$, i.e. $\nabla F(w_{*}) = 0$. Then, if $F$ is convex, then $w_{*} \in \arg \min_{w \in \mathbb{R}^d} F(w)$.
Consequently, for any permutation $\pi^{(t)}$ of $[n]$, we have
\begin{equation}\label{eq:fact1}
\sum_{j=0}^{n-1}\nabla{f}(w_{*}; \pi^{(t)}(j+1)) = 0.
\end{equation}
\item For any $1 \leq i \leq n$, from the update of $w_i^{(t)}$ in Algorithm~\ref{sgd_replacement}, we have
\begin{equation}\label{eq:fact2}
\arraycolsep=0.2em
\begin{array}{lcl}
w_i^{(t)} & = &  \tilde{w}_{t-1} - \frac{\eta_t}{n}\sum_{j=0}^{i-1} \nabla{f}(w_j^{(t)}; \pi^{(t)}(j+1)), \vspace{1ex}\\
\tilde{w}_t & = &  \tilde{w}_{t-1} - \frac{\eta_t}{n} \sum_{j=0}^{n-1} \nabla{f}(w_j^{(t)}; \pi^{(t)}(j+1)).
\end{array}
\end{equation}
\end{itemize}

\begin{lem}\label{le:ncvx_keybound1}
Suppose that Assumption \ref{ass_Lsmooth_fi} and Assumption~\ref{ass_general_bounded_variance} hold for \eqref{ERM_problem_01}. 
Let $\sets{w_i^{(t)}}$ be generated by  Algorithm~\ref{sgd_replacement} with any shuffling strategy $\pi^{(t)}$ and a learning rate $\eta_i^{(t)} := \frac{\eta_t}{n} > 0$ for a given positive sequence $\sets{\eta_t}$ such that $ 0 < \eta_t \leq \frac{1}{L\sqrt{3}}$. 
Then, we have
\begin{equation}\label{eq:ncvx_keybound1}
\sum_{j=0}^{n-1} \Vert w_j^{(t)} - w_0^{(t)} \Vert^2 \leq  n \eta_t^2 \cdot \left[ \left( 3 \Theta + 2 \right) \Vert   \nabla F ( w_0^{(t)}) \Vert^2 + 3 \sigma^2 \right].
\end{equation}
If $\pi^{(t)}$ is uniformly sampled at random without replacement from $[n]$ and the learning rate $\eta_t$ satisfies $0 < \eta_t \leq \frac{1}{L\sqrt{3}}$ for all $t \geq 1$, then we have
\begin{equation}\label{eq:ncvx_keybound1_reshuffling}
\mathbb{E}\Big[ \sum_{j=0}^{n-1} \Vert w_j^{(t)} - w_0^{(t)} \Vert^2 \Big]  \leq 2 \eta_t^2 \cdot \left[ \left(\Theta + n \right)\mathbb{E} \big[ \Vert   \nabla F ( w_0^{(t)}) \Vert^2 \big] +  \sigma^2 \right]. 
\end{equation}
\end{lem}

\begin{lem}[Lemma 5 in \cite{Nguyen2021ShufflingUnified}]
If $0 < \eta_t \leq \frac{1}{2L}$ for all $t \geq 1$, then we have 
\begin{equation}\label{eq_thm_weight_01}
    \frac{1}{n} \sum_{i=0}^{n-1} \norms{ w_{i}^{(t)} - w_{0}^{(t)} }^2  \leq \eta_t^2 \cdot \frac{8 L^2}{3} \norms{ w_{0}^{(t)} - w_{*} }^2 \ + \ \frac{16 L^2 \sigma_{*}^2}{3} \cdot \eta_t^4  \ + \ 2\sigma_{*}^2 \cdot \eta_t^2. 
\end{equation}
\end{lem}

\begin{thm}
Assumptions~\ref{ass_lowerbound_fi}, \ref{ass_Lsmooth_fi}, \ref{ass_PL_fi}, \ref{ass_general_bounded_gradient}, \ref{ass_general_bounded_weight}. Choose $\eta_t \leq \frac{1}{2L}$. 
\end{thm}

\begin{proof}
Analysis. For $i \in [n]$, we have
\allowdisplaybreaks
\begin{align*}
    f( w_0^{(t+1)} ; i )  & \overset{\eqref{eq:Lsmooth}}{\leq}   f( w_0^{(t)} ; i ) + \nabla f( w_0^{(t)} ; i )^{\top}(w_0^{(t+1)} - w_0^{(t)}) + \frac{L}{2}\norms{w_0^{(t+1)} - w_0^{(t)}}^2 \\
    %
    &\overset{\tiny\eqref{eq:fact2}}{=} f( w_0^{(t)} ; i ) - \eta_t \nabla f( w_0^{(t)} ; i )^\top \left( \frac{1}{n} \sum_{i=0}^{n-1} \nabla f (w_j^{(t)} ; \pi^{(t)} (j + 1) ) \right) \\ 
    & \qquad  + {~} \frac{L \eta_t^{2}}{2} \left \|  \frac{1}{n}\sum_{j=0}^{n-1} \nabla f (w_j^{(t)} ; \pi^{(t)} (j + 1) ) \right\|^2. \tagthis \label{eq_basic_001}
\end{align*}
% Averaging from $i = 1,\dots,n$ to both sides of \eqref{eq_basic_001}, we have
% \begin{align*}
%     F( w_0^{(t+1)} )  & \leq  F ( w_0^{(t)} ) - \eta_t \nabla F ( w_0^{(t)} )^\top \left( \frac{1}{n} \sum_{i=0}^{n-1} \nabla f (w_j^{(t)} ; \pi^{(t)} (j + 1) ) \right) \\ 
%     & \qquad  + {~} \frac{L \eta_t^{2}}{2} \left \|  \frac{1}{n}\sum_{j=0}^{n-1} \nabla f (w_j^{(t)} ; \pi^{(t)} (j + 1) ) \right\|^2 \\
%     %
%     & \overset{\tiny(a)}{=}   F( w_0^{(t)} ) - \frac{\eta_t}{2} \norms{ \nabla F( w_0^{(t)} ) }^2 + \frac{\eta_t}{2} \left \| \nabla F ( w_0^{(t)} )  - \frac{1}{n}\sum_{j=0}^{n-1} \nabla f (w_j^{(t)} ; \pi^{(t)} (j + 1) ) \right\|^2 \\
%     & \qquad  - {~} \frac{\eta_t}{2} \left( 1 - L\eta_t  \right) \left\| \frac{1}{n}\sum_{j=0}^{n-1} \nabla f (w_j^{(t)} ; \pi^{(t)} (j + 1) ) \right\|^2 \\
%     %
%     & \overset{\tiny(b)}{\leq} F( w_0^{(t)} ) - \frac{\eta_t}{2} \norms{ \nabla F( w_0^{(t)} ) }^2 \\ 
%     & \qquad + \frac{\eta_t}{2} \left \| \frac{1}{n}\sum_{j=0}^{n-1} \nabla f (w_0^{(t)} ; \pi^{(t)} (j + 1) )  - \frac{1}{n}\sum_{j=0}^{n-1} \nabla f (w_j^{(t)} ; \pi^{(t)} (j + 1) ) \right\|^2 \\
%     %
%     & \leq F( w_0^{(t)} ) - \frac{\eta_t}{2} \norms{ \nabla F( w_0^{(t)} ) }^2 \\ 
%     & \qquad + \frac{\eta_t}{2} \frac{1}{n}\sum_{j=0}^{n-1} \left \| \nabla f (w_0^{(t)} ; \pi^{(t)} (j + 1) )  - \nabla f (w_j^{(t)} ; \pi^{(t)} (j + 1) ) \right\|^2 \\
%     %
%     & \overset{\tiny\eqref{eq:Lsmooth_basic}}{\leq} F( w_0^{(t)} ) - \frac{\eta_t}{2} \norms{ \nabla F( w_0^{(t)} ) }^2 + \frac{\eta_t L^2}{2} \frac{1}{n}\sum_{j=0}^{n-1} \left \|  w_0^{(t)} - w_j^{(t)}  \right\|^2, \tagthis \label{eq_main_002}
% \end{align*}
% where (\textit{a}) follows from $u^{\top}v = \frac{1}{2}(\norms{u}^2 + \norms{v}^2 - \norms{u - v}^2)$; (\textit{b}) follows from the fact that $\eta_t \leq \frac{1}{L}$. 

Averaging from $i = 1,\dots,n$ to both sides of \eqref{eq_basic_001}, we have
\begin{align*}
    F( w_0^{(t+1)} )  & \leq  F ( w_0^{(t)} ) - \eta_t \nabla F ( w_0^{(t)} )^\top \left( \frac{1}{n} \sum_{i=0}^{n-1} \nabla f (w_j^{(t)} ; \pi^{(t)} (j + 1) ) \right) \\ 
    & \qquad  + {~} \frac{L \eta_t^{2}}{2} \left \|  \frac{1}{n}\sum_{j=0}^{n-1} \nabla f (w_j^{(t)} ; \pi^{(t)} (j + 1) ) \right\|^2 \\
    %
    & \overset{\tiny(a)}{=}   F( w_0^{(t)} ) - \frac{\eta_t}{2} \norms{ \nabla F( w_0^{(t)} ) }^2 + \frac{\eta_t}{2} \left \| \nabla F ( w_0^{(t)} )  - \frac{1}{n}\sum_{j=0}^{n-1} \nabla f (w_j^{(t)} ; \pi^{(t)} (j + 1) ) \right\|^2 \\
    & \qquad  - {~} \frac{\eta_t}{2} \left( 1 - L\eta_t  \right) \left\| \frac{1}{n}\sum_{j=0}^{n-1} \nabla f (w_j^{(t)} ; \pi^{(t)} (j + 1) ) \right\|^2 \\
    %
    & \overset{\tiny(b)}{\leq} F( w_0^{(t)} ) - \frac{\eta_t}{2} \norms{ \nabla F( w_0^{(t)} ) }^2 \\ 
    & \qquad + \frac{\eta_t}{2} \left \| \frac{1}{n}\sum_{j=0}^{n-1} \nabla f (w_0^{(t)} ; \pi^{(t)} (j + 1) )  - \frac{1}{n}\sum_{j=0}^{n-1} \nabla f (w_j^{(t)} ; \pi^{(t)} (j + 1) ) \right\|^2 \\
    & \qquad  - {~} \frac{\eta_t}{4} \left\| \frac{1}{n}\sum_{j=0}^{n-1} \nabla f (w_j^{(t)} ; \pi^{(t)} (j + 1) ) \right\|^2 \\
    %
    & \leq F( w_0^{(t)} ) - \frac{\eta_t}{2} \norms{ \nabla F( w_0^{(t)} ) }^2 \\ 
    & \qquad + \frac{\eta_t}{2} \frac{1}{n}\sum_{j=0}^{n-1} \left \| \nabla f (w_0^{(t)} ; \pi^{(t)} (j + 1) )  - \nabla f (w_j^{(t)} ; \pi^{(t)} (j + 1) ) \right\|^2 \\
    & \qquad  - {~} \frac{\eta_t}{4} \left\| \frac{1}{n}\sum_{j=0}^{n-1} \nabla f (w_j^{(t)} ; \pi^{(t)} (j + 1) ) \right\|^2 \\
    %
    & \overset{\tiny\eqref{eq:Lsmooth_basic}}{\leq} F( w_0^{(t)} ) - \frac{\eta_t}{2} \norms{ \nabla F( w_0^{(t)} ) }^2 + \frac{\eta_t L^2}{2} \frac{1}{n}\sum_{j=0}^{n-1} \left \|  w_0^{(t)} - w_j^{(t)}  \right\|^2 \\
    & \qquad  - {~} \frac{\eta_t}{4} \left\| \frac{1}{n}\sum_{j=0}^{n-1} \nabla f (w_j^{(t)} ; \pi^{(t)} (j + 1) ) \right\|^2 \\
    %
    & \overset{\tiny\eqref{eq:general_bounded_gradient_02}}{\leq} F( w_0^{(t)} ) - \frac{\eta_t}{2M} \frac{1}{n} \sum_{i=1}^n \norms{\nabla f(w_0^{(t)}; i) }^2 + \frac{\eta_t N}{2 M} [ F(w_0^{(t)}) - F_*] \\ & \qquad +  \frac{\eta_t L^2}{2} \frac{1}{n}\sum_{j=0}^{n-1} \left \|  w_0^{(t)} - w_j^{(t)}  \right\|^2 -  \frac{\eta_t}{4} \left\| \frac{1}{n}\sum_{j=0}^{n-1} \nabla f (w_j^{(t)} ; \pi^{(t)} (j + 1) ) \right\|^2, \tagthis \label{eq_main_003}
\end{align*}
where (\textit{a}) follows from $u^{\top}v = \frac{1}{2}(\norms{u}^2 + \norms{v}^2 - \norms{u - v}^2)$; (\textit{b}) follows from the fact that $\eta_t \leq \frac{1}{2L}$. 

Note that for $\alpha > 0$, we have
\begin{align*}
    & \frac{1}{1 + \alpha} \| a \|^2 - \frac{1}{\alpha} \| b \|^2 \leq \| a - b \|^2 \\
    & - \| a - b \|^2 \leq - \frac{1}{1 + \alpha} \| a \|^2 + \frac{1}{\alpha} \| b \|^2 \\
    & - \| b \|^2 \leq \alpha \| a - b \|^2 - \frac{\alpha}{\alpha + 1} \| a \|^2
\end{align*}

Adding $-F_*$ to both sides of \eqref{eq_main_003}, we have
\begin{align*}
    F( w_0^{(t+1)} ) - F_* & \leq [ F( w_0^{(t)} ) - F_*] - \frac{\eta_t}{2M} \frac{1}{n} \sum_{i=1}^n \norms{\nabla f(w_0^{(t)}; i) }^2 + \frac{\eta_t N}{2 M} [ F(w_0^{(t)}) - F_*] \\ & \qquad +  \frac{\eta_t L^2}{2} \frac{1}{n}\sum_{j=0}^{n-1} \left \|  w_0^{(t)} - w_j^{(t)}  \right\|^2
\end{align*}

\end{proof}

\subsection{New Result}

\begin{ass}\label{ass_new_property_fi}
Suppose that $f(\cdot; i)$ satisfies ABC inequality for some constant $M \in (1,+\infty)$ such that
\begin{equation}\label{eq:new_property_fi}
\norms{ \nabla f(w;i) - \nabla f(w_*;i) }^2 \leq M \langle \nabla f(w;i) - \nabla f(w_*;i), w - w_* \rangle , \quad \forall w \in \R^d, 
\end{equation}
where $w_*$ is a global solution of $F$. 
\end{ass}

Note that \eqref{eq:new_property_fi} implies $\norms{ \nabla f(w;i) - \nabla f(w_*;i) } \leq M \| w - w_* \|$, which is similar to $M$-smooth of $f(w;i)$, $i \in [n]$, if $w' = w_*$. 
Assumption~\ref{eq:new_property_fi} with Assumption~\ref{ass_PL_fi} (PL on each $f(w;i)$) and $\nabla f(w_*;i) = 0$, $i \in [n]$ imply
\begin{align*}
    2\mu [ \nabla f(w;i) - f_i^{*} ] \leq \norms{ \nabla f(w;i) }^2 \leq M \langle \nabla f(w;i), w - w_* \rangle
\end{align*}
which is equivalent to 
\begin{align*}
    \frac{2\mu}{M} [ \nabla f(w;i) - f_i^{*} ] \leq \langle \nabla f(w;i), w - w_* \rangle. 
\end{align*}

If $\frac{2\mu}{M} \geq 1$, then $f(w;i)$ is star-convex (at $w_*$). However, we consider the case $\frac{2\mu}{M} < 1$ which is non-convex. 

\begin{thm}\label{thm_convex_02}
Let $\{w^{(t)}_i\}$ be the sequence generated by Algorithm~\ref{sgd_replacement} with $\eta_i^{(t)} = \frac{\eta_t}{n}  = \frac{\eta}{n}$, with $0 < \eta \leq \frac{n}{M}$.
Then, under Assumptions~\ref{ass_lowerbound_fi}, \ref{ass_Lsmooth_fi}, \ref{ass_opt_set}, and \ref{eq:new_property_fi}, we have ...
\end{thm}

\begin{proof}
From the update $w_{i+1}^{(t)} := w_{i}^{(t)} - \eta_i^{(t)} \nabla f ( w_i^{(t)} ; \pi^{(t)} ( i + 1 ) )$ in Algorithm~\ref{sgd_replacement} with $\eta_i^{(t)} := \frac{\eta_t}{n}$,  for $i \in [n]$, we have
\begin{align*}
    w_{i}^{(t)} = w_{i-1}^{(t)} - \frac{\eta_t}{n} \nabla f ( w_{i-1}^{(t)} ; \pi^{(t)} (i)) = w_{0}^{(t)} - \frac{\eta_t}{n} \sum_{j=0}^{i-1} \nabla f ( w_{j}^{(t)} ; \pi^{(t)} (j + 1)). \tagthis \label{update_shuffling_01}
\end{align*}
Hence, 
\begin{align*}
    w_{0}^{(t+1)} = w_{n}^{(t)} = w_{0}^{(t)} - \frac{\eta_t}{n} \sum_{j=0}^{n-1} \nabla f ( w_{j}^{(t)} ; \pi^{(t)} (j + 1)). \tagthis \label{update_shuffling_02}
\end{align*}

For any $w^* \in W^*$, we have, 
\begin{align*}
    \| w_{i}^{(t)} - w^* \|^2 & \overset{\eqref{update_shuffling_01}}{=} \| w_{i-1}^{(t)} - w^* \|^2 - \frac{2 \eta_t}{n}\langle \nabla f ( w_{i-1}^{(t)} ; \pi^{(t)} (i)) , w_{i-1}^{(t)} - w^*  \rangle + \frac{\eta_t^2}{n^2} \| \nabla f ( w_{i-1}^{(t)} ; \pi^{(t)} (i))  \|^2 \\
    %
    &\overset{\eqref{eq:new_property_fi}}{\leq} \| w_{i-1}^{(t)} - w^* \|^2 - \frac{2 \eta_t}{M n} \| \nabla f ( w_{i-1}^{(t)} ; \pi^{(t)} (i))  \|^2 + \frac{\eta_t^2}{n^2} \| \nabla f ( w_{i-1}^{(t)} ; \pi^{(t)} (i))  \|^2 \\
    %
    & \leq \| w_{i-1}^{(t)} - w^* \|^2 - \frac{\eta_t}{Ln} \| \nabla f ( w_{i-1}^{(t)} ; \pi^{(t)} (i))  \|^2, 
\end{align*}
where the last inequality follows since $\eta_t \leq \frac{n}{M}$. Summing $i = 1,\dots,n$, we have
\begin{align*}
    \| w_{n}^{(t)} - w^* \|^2 & \leq \| w_{0}^{(t)} - w^* \|^2 - \frac{\eta_t}{M}  \frac{1}{n} \sum_{i=1}^{n} \| \nabla f ( w_{i-1}^{(t)} ; \pi^{(t)} (i))  \|^2 \leq \| w_{0}^{(t)} - w^* \|^2. \tagthis \label{eq_bounded_weight_01}
\end{align*}

Note that for $\alpha > 0$, we have \textbf{[DOUBLE CHECK]}
\begin{align*}
    & \frac{1}{1 + \alpha} \| a \|^2 - \frac{1}{\alpha} \| b \|^2 \leq \| a - b \|^2 \\
    & - \| a - b \|^2 \leq - \frac{1}{1 + \alpha} \| a \|^2 + \frac{1}{\alpha} \| b \|^2 \\
    & - \| b \|^2 \leq \alpha \| a - b \|^2 - \frac{\alpha}{\alpha + 1} \| a \|^2
\end{align*}

Note that $w_{n}^{(t)} = w_{0}^{(t+1)} = \tilde{w}_{t}$. From \eqref{eq_bounded_weight_01}, we also have
\allowdisplaybreaks
\begin{align*}
    \| w_{0}^{(t+1)} - w^* \|^2 & \leq \| w_{0}^{(t)} - w^* \|^2 - \frac{\eta_t}{M}  \frac{1}{n} \sum_{i=1}^{n} \| \nabla f ( w_{i-1}^{(t)} ; \pi^{(t)} (i))  \|^2 \\
    %
    & \overset{(a)}{\leq} \| w_{0}^{(t)} - w^* \|^2 - \frac{\alpha}{\alpha+1} \frac{\eta_t}{M}  \frac{1}{n} \sum_{i=1}^{n} \| \nabla f ( w_{0}^{(t)} ; \pi^{(t)} (i))  \|^2 \\
    & \qquad + \alpha \frac{\eta_t}{M}  \frac{1}{n} \sum_{i=1}^{n} \| \nabla f ( w_{i-1}^{(t)} ; \pi^{(t)} (i)) - \nabla f ( w_{0}^{(t)} ; \pi^{(t)} (i))  \|^2 \\
    %
    & \overset{\tiny\eqref{eq:Lsmooth_basic}}{\leq} \| w_{0}^{(t)} - w^* \|^2 - \frac{\alpha}{\alpha+1} \frac{\eta_t}{M}  \frac{1}{n} \sum_{i=1}^{n} \| \nabla f ( w_{0}^{(t)} ; \pi^{(t)} (i))  \|^2 \\
    & \qquad + \alpha \frac{\eta_t L^2}{M}  \frac{1}{n} \sum_{i=1}^{n} \| w_{i-1}^{(t)} - w_{0}^{(t)}  \|^2 \\
    % 
    & \overset{\tiny\eqref{eq_thm_weight_01}}{\leq} \| w_{0}^{(t)} - w^* \|^2 - \frac{\alpha}{\alpha+1} \frac{\eta_t}{M}  \frac{1}{n} \sum_{i=1}^{n} \| \nabla f ( w_{0}^{(t)} ; \pi^{(t)} (i))  \|^2 \\
    & \qquad + \alpha \frac{\eta_t^3 L^2}{M} \left(  \frac{8 L^2}{3} \norms{ w_{0}^{(t)} - w_{*} }^2 \ + \ \frac{16 L^2 \sigma_{*}^2}{3} \cdot \eta_t^2  \ + \ 2\sigma_{*}^2  \right) \\
    %
    &  \overset{\tiny\eqref{eq:PL_fi}}{\leq} \| w_{0}^{(t)} - w^* \|^2 - \frac{\alpha}{\alpha+1} \frac{2 \mu \eta_t}{M}  \frac{1}{n} \sum_{i=1}^{n} [ f ( w_{0}^{(t)} ; \pi^{(t)} (i)) - f_i^{*} ] \\
    & \qquad + \alpha \frac{\eta_t^3 L^2}{M} \left(  \frac{8 L^2}{3} \norms{ w_{0}^{(t)} - w_{*} }^2 \ + \ \frac{16 L^2 \sigma_{*}^2}{3} \cdot \eta_t^2  \ + \ 2\sigma_{*}^2  \right) \\
    %
    & \overset{\tiny\eqref{eq_loss_great_01}}{\leq} \| w_{0}^{(t)} - w^* \|^2 - \frac{\alpha}{\alpha+1} \frac{2 \mu \eta_t}{M}  [ F ( w_{0}^{(t)} ) - F_* ] \\
    & \qquad + \alpha \frac{\eta_t^3 L^2}{M} \left(  \frac{8 L^2}{3} \norms{ w_{0}^{(t)} - w_{*} }^2 \ + \ \frac{16 L^2 \sigma_{*}^2}{3} \cdot \eta_t^2  \ + \ 2\sigma_{*}^2  \right), \tagthis \label{eq_main_new_001}
\end{align*}
where $(a)$ follows since $- \| b \|^2 \leq \alpha \| a - b \|^2 - \frac{\alpha}{\alpha + 1} \| a \|^2$ for $\alpha > 0$. 

\end{proof}

